FloMo: Tractable Motion Prediction with Normalizing Flows

The future motion of traffic participants is inherently uncertain. To plan safely, therefore, an autonomous agent must take into account multiple possible trajectory outcomes and prioritize them. Recently, this problem has been addressed with generative neural networks. However, most generative models either do not learn the true underlying trajectory distribution reliably, or do not allow predictions to be associated with likelihoods. In our work, we model motion prediction directly as a density estimation problem with a normalizing flow between a noise distribution and the future motion distribution. Our model, named FloMo, allows likelihoods to be computed in a single network pass and can be trained directly with maximum likelihood estimation. Furthermore, we propose a method to stabilize training flows on trajectory datasets and a new data augmentation transformation that improves the performance and generalization of our model. Our method achieves state-of-the-art performance on three popular prediction datasets, with a significant gap to most competing models.

==> sections/normalizing_flows.tex <==
Normalizing flows are probabilistic models that can learn complex data distributions by transforming noise samples $\bfu$ from a simple base distribution $p_u(\bfu)$ into samples $\bfx$ from the target distribution:
\begin{equation}
\label{eq:flowtransform}
    \bfx = f(\bfu) \quad\text{where}\quad \bfu \sim p_u(\bfu).
\end{equation}
By defining the transformation $f(\bfu)$ such that it is invertibe and differentiable, the probability density of $\bfx$ can be obtained by a change of variables~\cite{papamakarios2019normalizing}:
\begin{equation}
\label{eq:flowforward}
    p_x(\bfx) = p_u(\bfu) {\left| \det \thinspace J_{f}(\bfu) \right|}^{-1}.
\end{equation}
Here $J_{f}(\bfu)$ denotes the Jacobian matrix of the function $f(\bfu)$. In the same manner, by the inverse function theorem, it is also possible to express $p_x(\bfx)$ in terms of $\bfx$ and $J_{f^{-1}}$:
\begin{equation}
\label{eq:flowinverse}
    p_x(\bfx) = p_u(f^{-1}(\bfx)) \left| \det \thinspace J_{f^{-1}}(\bfx) \right|.
\end{equation}
For the base distribution, usually a standard normal is chosen and the invertible transformation is implemented by a neural network. To make the flow more flexible, several such transformations can be composed. It is important that the Jacobian determinant can be computed efficiently and, depending on the use case, the flow must be easy to invert. Furthermore, to represent complex distributions the transformations in the flow must be expressive.
